Tree decomposition and parameterized algorithms for RNA structure-sequence alignment including tertiary interactions and pseudoknots

We present a general setting for structure-sequence comparison in a large class of RNA structures that unifies and generalizes a number of recent works on specific families on structures. Our approach is based on tree decomposition of structures and gives rises to a general parameterized algorithm, where the exponential part of the complexity depends on the family of structures. For each of the previously studied families, our algorithm has the same complexity as the specific algorithm that had been given before.

==> background-long.tex <==
\section{Background}

The many variants of the general problem of RNA sequence and structure comparison have several applications in bioinformatics. Notably, computing multiple structural sequence alignments provides a powerful approach for predicting the common structure of a set of RNA sequences~\cite{Gardner2005}, and structure-structure comparison allows to find local or global similarities between RNA structures (see {\it e.g.}~\cite{Hochsmann2003,Allali2005}), and to classify them into functional families~\cite{Allali2012}.

This paper focuses on pairwise sequence-structure comparison, that is comparing a RNA sequence with an unknown structure to a sequence whose structure is known.
This problem occurs in two main kinds of applications.
The first one is searching for a given structured RNA in a long sequence or a set of sequences.
Notably, searching for non-coding RNA genes in genomes may involve aligning a structural model of an RNA family to a long sequence, thus searching for a subsequence that has sequence and structure similarities with the family~\cite{Freyhult2007}.
The other application is tertiary structure prediction, or three-dimensional (3D) modeling, by homology.
In this case, the tertiary structure of an RNA molecule is known, and the problem is to precisely align one or several homologous sequences to the structured sequence  in order to  predict (at least partially) their structures. This problem is crucial because current {\it ab initio} approaches for RNA 3D modeling only handle sequences of a few dozens nucleotides~\cite{Das2007,Ding2008,Parisien2008}.
Predicting the 3D structure of large molecules involves combining {\it ab initio} and comparative approaches in interactive software where the process is guided  by the user step by step~\cite{Jossinet2010}.

For comparison purposes, an RNA structure is represented as a graph (or by an equivalent combinatorial structure called arc-annotated sequence, as will be seen below) whose nodes are nucleotides and edges represent interactions between them \cite{Bafna1995}.
In 2002, Jiang and his co-authors addressed the problem of pairwise comparison of RNA structures in its full generality~\cite{JiangLMZ02}.
To this purpose, they defined the edit distance problem on RNA structures, using a set of atomic edition operations that had been defined in~\cite{Evans1999a}.
Notably, they gave a dynamic programming algorithm in $\bigO(nm^3)$ time complexity for comparing a sequence to a  {\em nested} structure (in other words, a secondary structure without pseudoknots), where $n$ is the length of the sequence with known structure and $m$ the length of the sequence of unknown structure.
This complexity was later refined to $O(n_1m^2 + n_2m^3)$ in~\cite{Le2004}, where $n=n_1+n_2$ and where $n_2$ is the number of so-called {\em multiloops} in the structure.
They also established that computing the edit distance between a sequence and a structure is a NP-hard (and even Max-SNP-hard) problem if the structure is {\em crossing}, that is if it contains pseudoknots. (More general results on the computational complexity of RNA comparison are reported in~\cite{Blin2007,Blin2010}.)

Meanwhile, considering general structures, that is structures containing all the known interactions in RNAs including non-canonical ones~\cite{LW2001} and pseudoknots, is crucial for computing precise sequence-structure alignments.
In~\cite{JiangLMZ02}, a polynomial algorithm was developed for pseudoknotted structures, but it involves strong constraints on the costs of the edition operations.
The other approaches that have been developed up to now either are based on heuristics, or focus on restricted classes of pseudoknots.
As regards heuristics, a way to tackle with the intrinsic time complexity is to represent the structures at a much lower precision level, by considering structural elements (such as stems and loops) as the nodes of the structural graph.
%This allows to run hight polynomial or exponential algorithms on small graphs.
Notably, in~\cite{Song2006}, a dynamic programming approach has been developed over a tree decomposition of a coarse grained structure graph.
Other approaches aim to give near optimal solutions.
For example, in~\cite{Lenhof1998} the problem is changed into an integer linear program and solved by a branch-and-cut approach.
However, experiments show that this approach is not efficient in terms of computation time.
A similar representation is used in~\cite{Bauer2007,Bauer2008}, where Lagrangian relaxation is used to obtain a near optimal solution in more reasonable time.

It has been observed that the so-called {\em H-type} and {\em kissing-hairpin} pseudoknots represent more than $80\%$ of the pseudoknots in known structures~\cite{Rodland2006}.
When considering structures that contain only these kinds of pseudoknots, the problem can be solved in polynomial time with a complexity in $O(nm^4)$, or $O(nm^3)$ if only H-Type pseudoknots are allowed~\cite{Han2008,Wong2011}. Moreover, in~\cite{Han2008} these two classes of pseudoknots where embedded into a much more general class, the {\em standard pseudoknots} of degree $k$ (with $k=3$ for H-type pseudoknots and $k=4$ for kissing-hairpins). They gave the general idea to write algorithms in $O(nm^k)$ and $O(nm^{k+1})$, respectively, for a single standard pseudoknots, and for a standard pseudoknot which is embedded inside a terminal loop. Recently, the even more general class of simple non-standard pseudoknots of degree $k$ was defined, and an algorithm was given for handling such a pseudoknot,  in $O(nm^k)$ if alone, or in $O(nm^{k+1})$ for a simple recursion (a nested structure embedded in a simple non-standard pseudoknot  \cite{Wong2011}). Very recently, in~\cite{Wong2012} an algorithm in $O(nm^3)$ has been given for a class of structures involving triple helices, where a nucleotide can be paired to two other nucleotides.

In the present paper, we give a general setting for sequence-structure comparison in a large class of RNA structures that unifies and generalizes all the above families of structures.
Notably, we handle structures where each nucleotide can be paired to any number of other nucleotides, thus considering all kinds of non-canonical interactions~\cite{LW2001} and generalising the work in~\cite{Wong2012}. Our approach is based on {\em tree decomposition} of structures, where the degree of each pseudoknot is directly related to the {\em tree-width} of the decomposition. Table~\ref{tableComplex} gives a summary of the previous works that are generalized by our approaches, and the time complexity of our algorithm for each of the classes.

%%%%% Tableau recapitulatif des algo et complexitÃ© %%%%%%
\begin{table}[t]
{\centering \begin{tabular}{|p{6.3cm}|l|c|c|} \hline
Structures                                         & Time complexity &\rotatebox{70}{Base triples}&\rotatebox{70}{Reference(s)}\\ \hline
% Yann: Je prefere virer les $l*$, car plus lisible
%Secondary Structures (Pseudoknot-free)             & $O(lm^3+(n-l)m^2)$                & no  & \cite{Bafna1995}             \\ \hline
Secondary Structures (Pseudoknot-free)             & $O(lm^3+nm^2)$                & no  & \cite{Bafna1995}             \\ \hline
Standard Pseudoknots                              & $O(nm^k)$                         & no  & \cite{Han2008}             \\ \hline
%Embedded Standard Pseudoknots                     & $O(l_pm^k + lm^3 + (n-l_p-l)m^2)$ & no  & \cite{Han2008}             \\ \hline
Embedded Standard Pseudoknots                     & $O(l_pm^k + lm^3 + nm^2)$ & no  & \cite{Han2008}             \\ \hline
Simple Non-Standard Pseudoknots                   & $O(nm^{k+1})$                     & no  & \cite{Wong2011}             \\ \hline
2-Level Recursive Simple Non-Standard Pseudoknots & $O(nm^{k+2})$                     & no  & \cite{Wong2011}             \\ \hline
Triple Helices                                     & $O(nm^3)$                         & yes & \cite{Wong2012}             \\ \hline
Standard Structures                                & $O(nm^k)$                         & yes & $\times$                   \\ \hline
Recursive Standard Structures                      & $O(nm^{k+1})$                     & yes & $\times$              \\ \hline
Simple Non-Standard Structures                     & $O(nm^{k+1})$                     & yes & $\times$              \\ \hline
Recursive Simple Non-Standard Structures           & $O(nm^{k+2})$                     & yes & $\times$              \\ \hline
\end{tabular}\\}

\label{tableComplex}
\caption{Summary of existing algorithms for sequence structure comparison. Our approach unifies all these algorithms and, for each class of structures captured by pre-existing works, specializes into time complexities
that
%either
matches
%of improves over
previous efforts. Notations: $l$ is the number of helices implied in three way (or more) junctions;
$l_p$ is the length of the pseudoknot region;
$k$ is the degree of the pseudoknot/(simple) standard structure.}
\end{table}


The paper is organized as follows. In Section~\ref{} we define the sequence-structure alignment problem. In Section~\ref{} we define the tree decomposition of an arc-annotated sequence, and we present a general dynamic programming alignment algorithm between a structure which has been decomposed into a tree, and a sequence. We also give the complexity of the algorithm, according to the size of the sequence, the size of the structure, and the tree-width of the decomposition. In Section~\ref{}we present a general algorithm that computes a tree decomposition of a structure, provided that a so-called wave embedding of the structure is known. Then we show how it applies to all families of structures that had been studied up to now as well as more general families, as shown in  Table~\ref{tableComplex}.\Alain{Rappel : nous avons decide de fondre en une seule les sections 4 et 5}.

 % A supprimer aprÃ¨s utilisation :
  %Sequence structure alignment : \\
  %\begin{itemize}
   %\item Secondary Structure : $O(nm^3)$ \cite{JiangLMZ02,Bafna1995}  and $O(n_1m^2 + n_2m^3)$ \cite{Le2004}(with $n=n_1+n2$ and where $n_2$ is the number of multiloops).
    %     Note that \cite{JiangLMZ02,Bafna1995} is already in $O(n_1m^2 + n_2m^3)$ but not explain.
   %\item Standard PK  : $O(nm^k)$ \cite{Han2008} and $O(nm^{k+1})$ for embedded standard PK (an standard PK inside a terminal loop of a simple helix).
   %\item Simple non Standard PK  : $O(nm^k)$, with $k$ the degree of the PK (usually one more than the standard PK ``hidden'' in the Simple non standard PK ) (\cite{Wong2011}
%         and $O(nm^{k+1})$ for a simple recursion (a regular structure embedded in a Simple non Standard PK
%  \end{itemize}

%Sequence structure alignment : \\
%  Us : $O(nm^k)$ for standard structure of degree $k$ (include Standard PK of degree $k$).
%    $O(nm^{k+1})$ for recursive standard structure of degree $k$ (any level of recursion).
% In fact, it is more parametrized, the $+1$ depends of the parity of the degree of the standard structure.
%For example:  $O(n_1m^2 + n_2m^3)$ for secondary structure\dots{}


